Robust Constrained Multi-objective Evolutionary Algorithm based on Polynomial Chaos Expansion for Trajectory Optimization

An integrated optimization method based on the constrained multi-objective evolutionary algorithm (MOEA) and non-intrusive polynomial chaos expansion (PCE) is proposed, which solves robust multi-objective optimization problems under time-series dynamics. The constraints in such problems are difficult to handle, not only because the number of the dynamic constraints is multiplied by the discretized time steps but also because each of them is probabilistic. The proposed method rewrites a robust formulation into a deterministic problem via the PCE, and then sequentially processes the generated constraints in population generation, trajectory generation, and evaluation by the MOEA. As a case study, the landing trajectory design of supersonic transport (SST) with wind uncertainty is optimized. Results demonstrate the quantitative influence of the constraint values over the optimized solution sets and corresponding trajectories, proposing robust flight controls.

==> Intro_ver1.tex <==
\section{Introduction}
Multi-objective optimization is a common problem in the engineering field; it not only identifies a set of optimized solutions but also explicitly indicates the trade-off of multiple objective functions. Metaheuristic algorithms are effective for such optimization problems and have been widely used in the aerospace community, especially in the context of vehicle design \cite{Arias-Montano2012AeMOEA, Kanazaki2013airfoil, Kanazaki2016HybridRocket}. 

During the design optimization of a control sequence for aerospace vehicles, focus may need to be directed to the trade-off of multiple objective functions, rather than the detailed operational plans, such as the history of control or state transition during flights. However, in many cases, these objectives are highly coupled with the trajectory design. The coupling between high-fidelity aerodynamic properties and trajectory design is a critical problem, and the necessity for an efficient optimization method for the flight control system arises at the preliminary design phase\cite{Kanazaki2021SST, Tsuchiya2007MDO}. This issue is especially salient during the conceptual design of a new aircraft, where the empirical knowledge or global solutions for optimal design and control have not been investigated thoroughly. Supersonic transport (SST) design is one such example where such trade-offs must be taken into account.


The performance of landing and takeoff trajectories of an SST has a large correlation with the aerodynamic coefficients of the aircraft at low speed. However, since the airframe or wing shape of the SST is usually optimized for the cruising phase in a supersonic domain, a delta wing with a low aspect ratio is often selected; this causes limited available lift in the subsonic domain \cite{Razak1966}. Therefore, when performing the trajectory optimization with aerodynamic evaluation during the preliminary design phase, the influence of the vicissitude of the aerodynamic properties on the optimal control is not negligible. Therefore, the wind uncertainty must also be taken into account in the trajectory design. These uncertainties motivate robustness in the flight control during landing and takeoff, even for open-loop nominal control.

% Summing up the above discussion, designers of SST may expect robustness in control during the landing and takeoff, even for an open-loop nominal control; the multi-objective trajectory optimization which can deal with the robustness of time-series input with a compatible mathematical problem formulation and the efficient optimization method is desired. 
%However, since the consideration of robustness can often increase the number of constraints drastically, there has been a challenge of reducing the computational cost. 

In this study, an integrated robust multi-objective trajectory optimization method with constrained Multi-Objective Evolutionary Algorithm (MOEA) and non-intrusive Polynomial Chaos Expansion (PCE) is developed based on the coupled evaluation of aerodynamics and flight dynamics simulation. PCE is a widely used method for uncertainty quantification (UQ), which approximates the uncertainty of a certain variable with a linear combination of known orthogonal basis polynomials that take stochastic augments. By separating the constraints into the ones processed when generating the population, trajectory generation, and MOEA evaluation, robust multi-objective dynamic optimization with efficient constraint-handling is achieved. This optimization method is applied to the continuous descent operation (CDO) of the SST. %, where the robust solutions and the nominal solutions (i.e., no uncertainty) are compared. 

The contribution of this paper is twofold. First, we solve the robust multi-objective dynamic optimization problem with generalized constraints, while keeping its mathematical rigorousness. The robust formulation developed in \cite{Li2014PCE_RobTrajOpt} is expanded to a multi-objective problem, and the formulated problem is directly solved even though existing NLP-based methods are no longer applicable. This formulation evaluates the robustness based on probabilistic constraints rather than a tailor-made ``robustness index," which is expected in a wide range of applications.  
Secondly, we apply the method to trajectory design in a preliminary vehicle design, providing innovative insights into the robust design of the SST. 

The remainder of this paper proceeds as follows. Section \ref{LitReview} briefly reviews previous research on optimization methods concerning three key aspects: robustness, multi-objective problems, and aerospace trajectory design. Section \ref{Methodology} defines the generalized robust trajectory design problem and demonstrates the integrated optimization scheme. The SST landing trajectory design problem is introduced in Sec. \ref{SST_landing_formulation}. Finally, the results of the optimized trajectory design are examined in Section \ref{results}, and Section \ref{Conclusion} concludes this paper. 


\section{Literature Review} \label{LitReview}
In this paper, we focus on the intersection of three aspects of optimization: multi-objective optimization, robust optimization, and trajectory optimization. In this section, we summarize the literature that addresses these domains.

\subsection{Robustness in Trajectory Optimization}
In the field of trajectory optimization or path planning, numerous methods have been proposed to address uncertainty. Open-loop robust trajectories have been well investigated, and such trajectories can make the system less sensitive even without any feedback. 

One primary issue in this area of interest is making probabilistic constraints deterministic so that a deterministic optimization solver can deal with them in the minimum computational time possible. 
%One of the easiest and simplest implementations is an optimization method based on Monte-Carlo simulation \textcolor{red}{CITATION??}, while this usually ends up with intractable amount of computation. To reduce this large computational cost, a number of research directions have been sought. 
%One primary direction of such optimization method is an utilization of polynomial chaos \cite{Xiu2002PC, Eldred2008gPC}, which is a technique to estimate a random variable as a polynomial of another (simpler) random variable. This method is often adopted in the field of UQ, and also integrated into various trajectory optimization problems. \cite{Li2014PCE_RobTrajOpt, Matsuno2015conflict, Matsuno2016conflict, Fisher2011OptTrajGPC, Wang2019RobustConvex, Nakka2019Chanceconstr}.
The Uncertain Quantification (UQ) \cite{Luo2017survey} has been adopted in the trajectory optimization, and the utilization of Polynomial Chaos \cite{Xiu2002PC, Eldred2008gPC} has been demonstrated to be a convincing method among other techniques, such as linear covariance analysis \cite{Saunders2012OptTraj, Tang2007rendevous}, the Monte Carlo method \cite{Xu2014MC}, or ensemble prediction systems in meteorology \cite{Gonzalez2018RobustAircraft}, due to its high expressiveness and mathematical rigorousness \cite{Li2014PCE_RobTrajOpt, Matsuno2015conflict, Matsuno2016conflict, Fisher2011OptTrajGPC, Xiong2015PCE, Wang2019RobustConvex, Nakka2019Chanceconstr}.

% Another technique of capturing the uncertainty is linear covariance analysis, which addresses the uncertainty propagation of the linear system, often applied to the closed-loop GNC system \cite{Geller2006rendezvous}. Some paper proposed the robust trajectory optimization methods with this technique \cite{Saunders2012OptTraj, Tang2007rendevous}. 

% Also, an optimization method of aircraft trajectory planning based on ensemble prediction system, which predicts the probabilistic weather dynamics in  \cite{Gonzalez2018RobustAircraft}. 

A limitation of these studies is their focus on single-objective problems. In particular, integrating Nonlinear Programming (NLP)-based optimization methods, which are the primary methods for optimal control problems, into a multi-objective problem is nontrivial.

\subsection{Multi-objective Trajectory Optimization}

Multi-objective optimization of trajectory design has been gaining interest, mostly from air traffic management (ATM) researchers \cite{Gardi2016ATM_MO}, but also from the vehicle design community \cite{Fujikawa2015MDO, Kanazaki2021SST, Brevault2020MDO}; this is because trajectory design is highly coupled with the overall performance of the newly designed vehicles. Moreover, trade-off studies of multiple objectives are preferred in several other trajectory designs \cite{Zhang2013parafoil, Chai2016fuzzy, Morante2019MGA}.

% For most multi-objective trajectory design, the optimizer either merges multiple objectives into single objective based on weighted sum methods, or adopts population-based metaheuristics algorithms.  

% Moreover, the trade-off study of multiple objectives are preferred in some other trajectory designs. Luo, Tnag and Lei performed a rendezvous trajectory optimization problem via NSGA-II by setting the impulse time and impulse vector as design variables \cite{Luo2007MOrendezvous}. The homing trajectory of parafoil is optimized in \cite{Zhang2013parafoil}, based on the weighted-sum objective function and the Gaussian pseudospectral method, which converts the optimal control problem into a NLP. Similarly, Chai, Savvaris, and Tsourdos used fuzzy physical programming to bring multi-objective formulation into the single-objective formulation \cite{Chai2016fuzzy}. However, these methods require the tuning of the parameters when merging multiple objectives into one, which is a nontrivial process for the designers. 

% The EA and NLP are sequentially integrated to solve low-thrust multi-gravity-assist interplanetary trajectories in \cite{Morante2019MGA}. Chai et al. proposed the MOEA algorithm (NSGA-III) with three constraint handling methods, which qualitatively measures the constraint violation so that the entire optimization process will be facilitated even if the problem has a lot of constraints \cite{Chai2018EA}. 

The direct predecessor of this study is that of \cite{Kanazaki2021SST}, in which the authors performed optimization of the CDO for SST with MOEA. The high-fidelity aerodynamic analysis was approximated by a surrogate model, which reduced the computational cost while enabling the control optimization of the landing trajectory. However, the aerodynamic performance of many newly designed aircraft has high sensitivity, and consideration of uncertainty in these systems is yet to be addressed. 

\subsection{Robust Multi-objective Optimization}

Robustness towards stochastic scenarios is vital when pursuing pragmatic engineering designs. Research on robust optimization under uncertainty has been widely conducted \cite{Park2006RobustDesign, Du1999Robust}; the robustness in a multi-objective problem is of equal importance, however the difficulty increases due to its complexity \cite{Deb2006RobustMO}. 

Some studies integrated the MOEA and PCE successfully. The unique combination of the PCE and evolutionary algorithm (EA) for a robust static optimization problem using the ``meta-model," which replaces the analytical expression of the objective function with the design of experiment (DOE), was demonstrated in \cite{Gao2021PCEmo}. Additionally, Novaes et al. used a similar technique to tune the parameters of an electrophysiological model \cite{Novaes2019pceGA}. However, both of these studies used the PCE as an approximation of static functions; uncertainty propagation in dynamic equations would be more computationally expensive. 

\subsection{Towards Robust Multi-Objective Trajectory Optimization}

Marto and Vasile proposed an optimization method for the robust multi-objective problem with epistemic uncertainty using surrogate modeling, where the objective was the lower expectation \cite{Marto2021MOtraj}. However, the solution can be too conservative if interested in probability distributions. References \cite{Luo2007MOrendezvous, Luo2014robust, Yang2017robust} defined an index of robustness, which was regarded as one objective. However, such arbitrary ``robustness metrics" are difficult to generalize and apply directly to other problems. A multi-objective dynamic aircraft path planning problem with wind uncertainty was solved in \cite{Gonzalez2019Aircraft}, however this study also included an index of robustness as an objective. Moreover, the proposed algorithm integrated the constraints in a unique way such that the treatment of the constraints could not been generalized. In particular, path constraints are were considered in the paper. 

The optimization method developed in the present paper directly solves the robust formulation developed in \cite{Li2014PCE_RobTrajOpt}. This formulation is derived from the general form of the deterministic trajectory optimization problem, where mathematical rigorousness is guaranteed, and can be applied to various general trajectory optimization problems without requiring additional elements, such as the introduction of a ``robustness index," which is oftentimes very specific to the problem. 
%The PCE-based transformations of the stochastic dynamic constraints are then integrated to the constrained MOEA, which can deal with both multiple objectives and probabilistic constraints. This can be applied to more general trajectory optimization problems in the sense that (1) trajectory optimization problems have a number of constraints including path constraints, and (2) constraints are explicitly expressed in terms of means and standard deviation, which makes the problem easier to be examined in various scenarios of uncertainty.

==> Intro_ver2.tex <==
Uncertainty in optimization is critical to solving real-world problems, however the integration of such probabilistic aspects makes the problems drastically challenging compared to nominal ones. In spite of extensive efforts to treat probabilistic expressions deterministically, much less research on multi-objective problems can be found compared to single-objective cases. 

Furthermore, the introduction of a dynamical system exacerbates the complexity, as the number of the constraints that have to be addressed, which includes not only the dynamics itself but also the state or control constraints over the time horizon, is multiplied by the discretized time steps. State-of-the-art constraint-handling techniques are unable to directly process such a plethora of constraints, especially for a multi-objective context. 

One real-world application of such a problem is a robust landing trajectory design of supersonic transport (SST) or civilian supersonic aircraft, where the uncertain vicissitude of wind or aerodynamic properties can severely influence its flight control. This is because the wing shapes of supersonic aircraft are usually optimized based on the performance in the trans/supersonic domain, resulting in a limited lift in the subsonic domain. This motivates robustness in the flight control during landing and takeoff, even for open-loop nominal control.  

\subsection{Contribution}
In this study, we propose an integrated method based on constrained multi-objective evolutionary algorithm (MOEA) and non-intrusive polynomial chaos expansion (PCE) to solve a robust multi-objective constrained trajectory optimization problem. PCE is a widely used method for uncertainty quantification (UQ); it approximates an uncertainty through the mapping of known orthogonal basis polynomials. 
By separating the constraints into the ones considered, processed, and evaluated when generating the population, trajectory, and MOEA, respectively, robust multi-objective trajectory optimization with efficient constraint handling is achieved. 
Note that we only focus on the open-loop control in the present study. 

The contribution of this paper is threefold. 
First, we set up a robust multi-objective trajectory optimization problem with generalized constraints while keeping its mathematical rigorousness; the robust formulation developed in \cite{Li2014PCE_RobTrajOpt} is expanded to a multi-objective problem.
Secondly, we develop the generalized constraint handling scheme to the formulated problem through the unique integration of the PCE and MOEA, which the existing NLP-based methods can no longer handle in the multi-objective case. This method can be applied to various multi-objective optimal control problems without any additional modifications. 
Finally, we apply the method to trajectory design in a preliminary vehicle design context, providing innovative insights into the robust design of the SST. 

\subsection{Related work}
% Robust Multi-objective Optimization
The robust optimization method has been widely used \cite{Park2006RobustDesign, Du1999Robust}, as considering stochastic scenarios is vital for pragmatic engineering design. The complexity increases when changing from a single-objective to a multi-objective problem \cite{Deb2006RobustMO, ide2016robustness, gaspar2008robustness}. A dynamic optimization problem (DOP) considers time-variable parameters instead of the autonomous dynamical system (i.e., equations of motion). Even though this is generally categorized as a different problem from that of trajectory optimization, several studies have been conducted to address the robust multi-objective cases \cite{GUO2019MOO,Xin2010RobustOpt,Guo2018MOvehicle,jin2013framework}.

% Uncertainty in Trajectory Optimization
In the field of trajectory optimization or path planning, numerous methods have been proposed to address uncertainty. Open-loop robust trajectories have been well investigated, and such trajectories can make the system less sensitive even without feedback. One primary interest in this area is making probabilistic constraints deterministic so that a deterministic optimization solver can deal with them in the minimum computational time possible. The UQ \cite{Luo2017survey} has been adopted in trajectory optimization, and the utilization of Polynomial Chaos \cite{Xiu2002PC, Eldred2008gPC} has been demonstrated to be a convincing method among other techniques, such as linear covariance analysis \cite{Saunders2012OptTraj, Tang2007rendevous}, the Monte Carlo method \cite{Xu2014MC}, or ensemble prediction systems \cite{Gonzalez2018RobustAircraft}, due to its high expressiveness and mathematical rigorousness \cite{Li2014PCE_RobTrajOpt, Matsuno2015conflict, Matsuno2016conflict, Fisher2011OptTrajGPC, Xiong2015PCE, Wang2019RobustConvex, Nakka2019Chanceconstr}. A limitation of these studies is their focus on single-objective problems. In particular, integrating Nonlinear Programming (NLP)-based optimization methods, which are the primary methods for single-objective optimal control problems, into a multi-objective problem is nontrivial.

% Multi-objective Trajectory Optimization
In the aerospace field, multi-objective trajectory optimization has been gaining interest, mostly from air traffic management (ATM) researchers \cite{Gardi2016ATM_MO}, but also from the vehicle design community \cite{Fujikawa2015MDO, Kanazaki2021SST, Brevault2020MDO}; this is because trajectory design is highly coupled with the overall performance of the newly designed vehicles. Moreover, trade-off studies of multiple objectives are preferred in several other trajectory designs \cite{Zhang2013parafoil, Chai2016fuzzy, Morante2019MGA}. The direct predecessor of this study is that of \cite{Kanazaki2021SST}, in which the authors performed optimization of the continuous descent operation (CDO) for SST with MOEA. The high-fidelity aerodynamic analysis was approximated by a surrogate model called the Kriging method, which reduced the computational cost while enabling the control optimization of the landing trajectory. Even though the aerodynamic performance of many newly designed aircraft has high sensitivity, the consideration of the uncertainty in the system is yet to be addressed.

% Robust  Multi-objective traj. optimization
Some studies have solved a robust multi-objective trajectory optimization problem. 
Marto and Vasile proposed an optimization method for the robust multi-objective problem with epistemic uncertainty using surrogate modeling, where the objective was lower expectation \cite{Marto2021MOtraj}. However, if we are interested in the probability distributions, the solution will be too conservative. 
References \cite{Luo2007MOrendezvous, Luo2014robust, Yang2017robust, Gonzalez2019Aircraft} defined the problem-specific indices of robustness, which was regarded as one objective. However, such tailor-made ``robustness metrics" are difficult to generalize and apply directly to other problems. 
A multi-objective dynamic aircraft path planning problem with wind uncertainty was solved in \cite{Gonzalez2019Aircraft}, however the proposed algorithm integrated the constraints in a unique way such that the treatment of the constraints could not be generalized. In particular, path constraints were not considered in the paper. 


\subsection{Paper organization}
The remainder of this paper is organized as follows. Section \ref{Methodology} defines the generalized robust multi-objective trajectory design problem and demonstrates the integrated optimization scheme. The SST landing trajectory design problem is introduced in Sec. \ref{SST_landing_formulation}. The results of the optimized trajectory are examined in Section \ref{results}, and Section \ref{Conclusion} concludes this paper. 

==> Tables/Noninf_numbers.tex <==
\begin{table}[ht]
\caption{Number of noninferior solutions of the optimization results}
\label{noninf_numbers_table}
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Scenario} & \textbf{\# of Solutions} \\
\hline
$\sigma_1 = 1.0$, $\sigma_2 = 150$ & 11145 \\
$\sigma_1 = 3.0$, $\sigma_2 = 150$ (Baseline) & 9409 \\
$\sigma_1 = 5.0$, $\sigma_2 = 150$ & 8751 \\
$\sigma_1 = 3.0$, $\sigma_2 = 100$ & 8748 \\
$\sigma_1 = 3.0$, $\sigma_2 = 200$ & 11694 \\
Deterministic & 25013 \\
\hline
\end{tabular}
\end{table} 

==> Tables/algo_param.tex <==
\begin{table}[htbp]
\caption{Key parameter values for algorithm implementation}
\label{algo_para}
\begin{center}
\begin{tabular}{|c|c|}
\hline
\textbf{Parameter}&\textbf{Value} \\
\hline
Generation, \# & 1200  \\
Number of population, \# & 30  \\
$\Delta t$, s & 0.1  \\
Number of Rudder angle manipulation, \#/s & 2 \\
\hline
\end{tabular}
\label{tab1}
\end{center}
\end{table}

==> Tables/comp_time.tex <==
\begin{table}[ht]
\caption{Time required for computation for different scenarios}
\label{comp_time}
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Scenario} & \textbf{Comp. Time, s} \\
\hline
$\sigma_1 = 1.0$, $\sigma_2 = 150$ &  \\
$\sigma_1 = 3.0$, $\sigma_2 = 150$ (Baseline) &  \\
$\sigma_1 = 5.0$, $\sigma_2 = 150$ &  \\
$\sigma_1 = 3.0$, $\sigma_2 = 100$ & 3354 \\
$\sigma_1 = 3.0$, $\sigma_2 = 200$ & 3721 \\
Deterministic &  \\
\hline
\end{tabular}
\end{table}
